A min-max regret approach for the Steiner Tree Problem with Interval Costs

Let G=(V,E) be a connected graph, where V and E represent, respectively, the node-set and the edge-set. Besides, let Q \subseteq V be a set of terminal nodes, and r \in Q be the root node of the graph. Given a weight c_{ij} \in \mathbb{N} associated to each edge (i,j) \in E, the Steiner Tree Problem in graphs (STP) consists in finding a minimum-weight subgraph of G that spans all nodes in Q. In this paper, we consider the Min-max Regret Steiner Tree Problem with Interval Costs (MMR-STP), a robust variant of STP. In this variant, the weight of the edges are not known in advance, but are assumed to vary in the interval [l_{ij}, u_{ij}]. We develop an ILP formulation, an exact algorithm, and three heuristics for this problem. Computational experiments, performed on generalizations of the classical STP instances, evaluate the efficiency and the limits of the proposed methods.

==> cronograma.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\centering
\caption{Cronograma de execução do projeto de pesquisa. O cronograma é dividido em 12 trimestres, resultando em uma pesquisa de 3 anos.}
\label{tab:cronograma}
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
             & \multicolumn{4}{c}{Ano 1} & \multicolumn{4}{c}{Ano 2} & \multicolumn{4}{c}{Ano 3} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(l){10-13}
             & 1         & 2         & 3         & 4         & 1         & 2         & 3         & 4         & 1         & 2         & 3         & 4 \\ \midrule
Atividade 1  & x &           &           &   &  x        &           &           & x &           &           &           & \\
Atividade 2  & x & x & x &           &           &           &           &        & x         &           &           & \\
Atividade 3  &   & x & x &           &           &           &           &           &           &           &           & \\
Atividade 4  &   & x & x &           &           &           &           &        &           &           &           & \\
Atividade 5  &           &           &           & x & x &        &           &           &           &           &           & \\
Atividade 6  &           &           &           &           & x & x & x &  x     &           &           &           & \\
Atividade 7  &           &           &           &           &   & x & x &  x        &           &           &           & \\
Atividade 8  &           &           &           &           &           &           & x & x &  x        &           &           & \\
Atividade 9  &           &           & x & x &           &           & x &           & x & x & x & x \\ \bottomrule
\end{tabular}
\end{table}

==> tables/results_c.tex <==
\begin{table}[!t] 
\caption{Resultados do L-Shaped Method para as instâncias C1}
\label{table:resultados_c} 
\centering 
\begin{tabular}{
  c % |V'|
  c % |I|
  c % inteiro
  c % otimo
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(3)] % gap
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(2)] % cortes
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=4.1(5)] % tempo estagio 1
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(4)] % tempo estagio 2
}
\toprule 
$|V'|$ & $|I|$ & inteira & otima & \mc{gap (\%)} & \mc{cortes} & \mc{$t_1$ (s)} & \mc{$t_2$ (s)} \\ \midrule 
\multirow{4}{*}{25} & 2 & 5 & 5 & 0.0(0)    & 8.4(53)  & 253.1(5375)   & 2.9(18)   \\ 
                    & 3 & 5 & 5 & 0.0(0)    & 10.6(69) & 15.4(93)      & 9.7(69)   \\ 
                    & 4 & 5 & 5 & 0.0(0)    & 3.6(30)  & 15.1(205)     & 12.5(171) \\ 
                    & 5 & 5 & 4 & 0.0(0)    & 2.4(5)   & 13.3(54)      & 12.8(50)  \\ 
\midrule 
\multirow{4}{*}{50} & 2 & 1 & 0 & 80.3(440) & 3.0(56)  & 3600.0(00)    & 22.6(482)  \\ 
                    & 3 & 1 & 0 & 80.3(441) & 1.6(25)  & 3600.0(00)    & 30.5(597)  \\ 
                    & 4 & 3 & 3 & 40.0(548) & 1.4(13)  & 1521.6(18800) & 43.1(541)  \\ 
                    & 5 & 1 & 1 & 80.0(447) & 1.4(21)  & 3201.7(12551) & 86.9(1400) \\ 
\bottomrule 
\end{tabular} 
\end{table} 


==> tables/results_r.tex <==
\begin{table}[!t] 
\caption{Resultados do L-Shaped Method para as instâncias R1}
\label{table:resultados_r} 
\centering 
\begin{tabular}{
  c % |V'|
  c % |I|
  c % inteiro
  c % otimo
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=3.1(3)] % gap
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(2)] % cortes
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=4.1(5)] % tempo estagio 1
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(3)] % tempo estagio 2
}
\toprule 
$|V'|$ & $|I|$ & inteira & ótima & \mc{gap (\%)} & \mc{cortes} & \mc{$t_1$ (s)} & \mc{$t_2$ (s)} \\ \midrule 
\multirow{4}{*}{25} & 2 & 1 & 1 & 80.0(447) & 1.4(9)   & 75.7(751)     & 0.4(7) \\ 
                    & 3 & 1 & 1 & 80.0(447) & 3.2(49)  & 81.3(652)     & 5.7(116) \\ 
                    & 4 & 1 & 1 & 80.0(447) & 2.4(31)  & 307.6(5750)   & 11.3(196) \\ 
                    & 5 & 5 & 5 & 0.0(0)    & 17.8(87) & 2789.4(22874) & 298.6(4372) \\ 
\midrule 
\multirow{4}{*}{50} & 2 & 0 & 0 & 100.0(0)  & 0.0(0)   & 3600.0(00)    & 0.0(0) \\ 
                    & 3 & 0 & 0 & 100.0(0)  & 0.0(0)   & 3600.0(00)    & 0.0(0) \\ 
                    & 4 & 0 & 0 & 100.0(0)  & 0.0(0)   & 3600.0(00)    & 0.0(0) \\ 
                    & 5 & 0 & 0 & 100.0(0)  & 0.0(0)   & 3600.0(00)    & 0.0(0) \\ 
\bottomrule 
\end{tabular} 
\end{table} 


==> tables/results_rc.tex <==
\begin{table}[!t] 
\caption{Resultados do L-Shaped Method para as instâncias RC1}
\label{table:resultados_rc} 
\centering 
\begin{tabular}{
  c % |V'|
  c % |I|
  c % inteiro
  c % otimo
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=3.1(3)] % gap
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(3)] % cortes
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=4.1(5)] % tempo estagio 1
  S[separate-uncertainty, table-align-uncertainty, table-number-alignment=center, table-format=2.1(3)] % tempo estagio 2
}
\toprule 
$|V'|$ & $|I|$ & inteira & ótima & \mc{gap (\%)} & \mc{cortes} & \mc{$t_1$ (s)} & \mc{$t_2$ (s)} \\ \midrule 
\multirow{4}{*}{25} & 2 & 3 & 2 & 41.5(535) & 12.2(126) & 1309.3(20758) & 4.1(46) \\ 
                    & 3 & 3 & 2 & 41.0(539) & 10.0(97)  & 984.2(20253)  & 8.7(92) \\ 
                    & 4 & 3 & 2 & 40.7(541) & 11.4(132) & 966.0(19114)  & 27.0(354) \\ 
                    & 5 & 5 & 5 & 0.0(0)    & 7.4(52)   & 113.2(1141)   & 72.0(750) \\ 
\midrule 
\multirow{4}{*}{50} & 2 & 0 & 0 & 100.0(0)  & 0.0(0)    & 3600.0(00)    & 0.0(0) \\ 
                    & 3 & 0 & 0 & 100.0(0)  & 0.0(0)    & 3600.0(00)    & 0.0(0) \\ 
                    & 4 & 1 & 0 & 82.9(382) & 0.4(9)    & 3600.0(00)    & 39.4(880) \\ 
                    & 5 & 0 & 0 & 100.0(0)  & 0.0(0)    & 3600.0(00)    & 0.0(0) \\ 
\bottomrule 
\end{tabular} 
\end{table} 

